A Modeling Framework for Schedulability Analysis of Distributed Avionics Systems

This paper presents a modeling framework for schedulability analysis of distributed integrated modular avionics (DIMA) systems that consist of spatially distributed ARINC-653 modules connected by a unified AFDX network. We model a DIMA system as a set of stopwatch automata (SWA) in UPPAAL to analyze its schedulability by classical model checking (MC) and statistical model checking (SMC). The framework has been designed to enable three types of analysis: global SMC, global MC, and compositional MC. This allows an effective methodology including (1) quick schedulability falsification using global SMC analysis, (2) direct schedulability proofs using global MC analysis in simple cases, and (3) strict schedulability proofs using compositional MC analysis for larger state space. The framework is applied to the analysis of a concrete DIMA system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{150}
\providecommand{\publicationstatus}{John P. Gallagher, Rob van Glabbeek and Wendelin Serwe (Eds):\\
Models for Formal Analysis of Real Systems (MARS'18)\\
and Verification and Program Transformation (VPT'18)
\\
EPTCS 268, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.268.5}{10.4204/EPTCS.268.5}}

